Optimization's Neglected Normative Commitments

Optimization is offered as an objective approach to resolving complex, real-world decisions involving uncertainty and conflicting interests. It drives business strategies as well as public policies and, increasingly, lies at the heart of sophisticated machine learning systems. A paradigm used to approach potentially high-stakes decisions, optimization relies on abstracting the real world to a set of decision(s), objective(s) and constraint(s). Drawing from the modeling process and a range of actual cases, this paper describes the normative choices and assumptions that are necessarily part of using optimization. It then identifies six emergent problems that may be neglected: 1) Misspecified values can yield optimizations that omit certain imperatives altogether or incorporate them incorrectly as a constraint or as part of the objective, 2) Problematic decision boundaries can lead to faulty modularity assumptions and feedback loops, 3) Failing to account for multiple agents' divergent goals and decisions can lead to policies that serve only certain narrow interests, 4) Mislabeling and mismeasurement can introduce bias and imprecision, 5) Faulty use of relaxation and approximation methods, unaccompanied by formal characterizations and guarantees, can severely impede applicability, and 6) Treating optimization as a justification for action, without specifying the necessary contextual information, can lead to ethically dubious or faulty decisions. Suggestions are given to further understand and curb the harms that can arise when optimization is used wrongfully.

==> sections/abtract.tex <==
Optimization is offered as an objective approach to resolving complex, real-world decisions involving uncertainty and conflicting interests. It drives business strategies as well as public policies and, increasingly, lies at the heart of sophisticated machine learning systems. A paradigm used to approach potentially high-stakes decisions, optimization relies on abstracting the real world to a set of \textit{decision(s)}, \textit{objective(s)} and \textit{constraint(s)}. Drawing from the modeling process and a range of actual cases, this paper describes the normative choices and assumptions that are necessarily part of using optimization. It then identifies six emergent problems that may be neglected: 1) {Misspecified values} can yield optimizations that omit certain imperatives altogether or incorporate them incorrectly as a constraint or as part of the objective, 2) {Misleading decision boundaries} can lead to faulty modularity assumptions, 3) {Failing to account for multiple agents}' divergent goals and decisions can lead to policies that serve only certain narrow interests, 4) {Label mismeasurement} can introduce bias and imprecision, 5) {Faulty use of relaxation and approximation} methods, unaccompanied by formal characterizations and guarantees, can severely impede applicability, and 6) {Treating optimization as a justification} for action, without specifying the necessary contextual information, can lead to ethically dubious or faulty decisions. Suggestions are given to further understand and curb the harms that can arise when optimization is used wrongfully.

==> sections/acknowledgements.tex <==
%\section*{Acknowledgments}
\begin{acks}
We thank the Digital Life Initiative (DLI), the AI, Policy and Practice Initiative (AIPP), the Cornell Tech Emma Pierson and Nikhil Garg (CTEN) Lab, and the Cornell University Information Science Colloquium for providing remarks and suggestions. We'd like to acknowledge Nikhil Garg, David Williamson, Yonatan Mintz, Eugene Bagdasaryan, Jon Kleinberg, and Karen Levy for providing invaluable feedback.

The authors are grateful for awards from the US National Science Foundation, NSF CNS-1704527 and the John D. and Catherine T. MacArthur Foundation, which generously supported this work. 
\end{acks}


==> sections/assumptions.tex <==
\subsection*{Choices, Abstractions and Assumptions}\label{sec:assumptions}

Formulating an optimization problem requires transforming complex information in the world into a simplified model. Models of any sort can (ideally) use abstraction and representation to make information communicable, actionable or useful \cite[p 20]{o2016weapons}. Therefore, models that are useful often omit or collapse a significant amount of information.

The idea of abstraction is familiar to computer scientists, whose introductory computer science classes often involve creating a simple \textit{class} or \textit{object} such as a `Bank Account' or an `Employee' (see e.g. \cite[p 316-319]{sommerville_2004}). Doing so does not involve building a physical bank, of course; instead students simply define a set of variables (such as name and salary) and functions (such as ``retire” or ``promote”). By removing significant material and contextual aspects of a real-world system, a computer program can simulate a few key functions in order to make a particular point or perform a particular task. Abstraction is powerful and crucial to the field of computing; however, it also poses challenges: through making assumptions and collapsing information, models risk misrepresenting or omitting key information.

In the following sections, we trace the component steps that constitute the optimization process. The process spans modeling, measurement, solving, and deploying, as shown in Figure \ref{fig:lifecycle}. Reasoning about these components requires assumptions--some axiomatic, others readily contestable. By systematically enumerating and formalizing these as constitutive parts of the optimization life cycle, the system's risks, harms and indeterminacies\footnote{In using assumptions, indeterminacies and \textit{vague} aspects of socio-technical systems to explore their normative implications, this paper draws inspiration from \citet{dobbe2021hard}.} can be more easily identified and communicated,\footnote{We do not claim to provide an exhaustive method for anticipating future harms or \textit{verifying} optimizations--such an endeavor eludes computer scientists. Our project is influenced by \citet{smith1985limits} on this matter: we seek to disambiguate and excavate the social and political aspects of optimization as a method, rather than make grand claims about its use.} and concealed normative positions can be identified.

\subsection{Modeling} \label{subsec:model}

A preliminary step in putting forward an optimization model is defining the set of variables and parameters that will be included in the model. These variables are then used to formalize the objective function, decision variable and constraints which together define the feasible set of potential decisions and their corresponding utility or performance. As the model is defined and worked with, modeling choices play a determining role in the larger optimization process and any resulting decisions.

In this section, we focus on the three components of a standard optimization and discuss the negotiable decisions and assumptions at play during the modeling process. We refer to Appendix \ref{app:opt} for the standard form of an optimization problem.

\subsubsection*{The Objective Function}  Specifying an objective function, utility function or goal immediately invokes values judgements. Formalizing an objective function often means relying on quantifiable notions of utility or welfare that are relevant for a given decision. Formalization of this sort can also involve omitting values or desiderata from consideration. When multiple goals are valuable to consider, modeling assumptions are needed to incorporate these goals into a single objective. Often, this process involves defining a \textit{welfare function}, a term borrowed from economics (see e.g. \cite{kaneko1979nash, coleman1966possibility}). Instantiating an objective of this sort typically involves weighing the relative importance of different goals, and characterizing the overall objective function’s mathematical properties, like whether it is convex \cite{boyd2004convex}. 

\subsubsection*{The Decision Variable} Specifying the decision variable(s) requires making a number of assumptions about the decision-making agent and their degree of control. The optimization paradigm presumes that a decision-maker has a certain set of options, and inquiry is narrowed to only comparing between the options. Such an approach avoids thorny questions about who is in control and whether they ought to be. Consider, for example, an optimization aimed at setting a regulatory fine. Defining the decision mathematically may necessarily involve stripping away particularities about how fines result from complex bureaucratic and deliberative processes. Instead, an optimization might model the decision simply as a single variable representing the dollar value of a fine. Abstractions of this sort can appear self-evident even as they conceal choices with decisive normative commitments.

\subsubsection*{The Constraints}. Specifying constraints is also known as specifying the \textit{feasible set} of decisions. This step involves making assumptions about the physical relationship between variables. For instance, an optimization problem may try to maximize production subject to a budgetary constraint. Budgets often play into optimizations and models must specify what kind of scarcity exists and how it is being measured: is the agent constrained monetarily? spatially? temporally? Though the feasible decision space is traditionally conceived of as the set of possible decisions, constraints are often used to guarantee that a decision meets some baseline ethical or social standard. We call these sorts of constraints \textit{values-driven constraints}, and note that \textit{fairness} is a particularly common values-driven desideratum that gets modeled as a constraint.\footnote{\citet{passi2019problem} discuss problem formulation and modeling in the context of fairness.} Section \ref{subsubsec:mistakenlymodelingconstraint} includes a more in-depth discussion of the modeling assumptions involved in incorporating values into an optimization's constraints.

\subsection{Operationalization, Measurement and Quantification} \label{subsec:measure}

Applying optimization requires a number of decisions aimed at \textit{relating an abstract quantity to the external world}. Where modeling (discussed in Section \ref{subsec:model}) involves modes of knowledge aimed at making sense of the chaos of the world, measurement is how we empirically find new information or physically instrument the world. There is significant work on the elusive nature of measurement---here we highlight theoretical groundwork \cite{barad2003posthumanist, joslyn2001semiotics, finkelstein1984review, jacobs2021measurement, moss2021objective} as well as technical work on bias in measurement \cite{obermeyer2019dissecting, millsap1993methodology, hernan2009invited, bhatt2021uncertainty}. In this section we categorize optimization's measurement assumptions into two categories: 1) defining what is being measured and 2) deciding how to measure it.\bldelete{ The reason we separate the two questions which are notoriously hard to disentangle\footnote{It is a long-studied phenomenon that measurement can alter the notion of what it is being measured: See, for instance, \cite{mackenzie2008engine}.\blcomment{add references}} arises from the syntactic format of the optimization problem: formally defining the variables, an optimization necessarily specifies exactly which quantities are relevant, and what connection they have to the real world.}

\textit{What is being measured?} Deciding what is relevant or worthwhile to measure is an impactful step in setting up an optimization model. When written out on paper, an optimization has finite number of variables, and the definitions of these variables are often formally listed. These variables constitute a highly abstracted and stylized version of the world---few of their characteristics may correspond to the real-world entity that they try to mimic or count. For example, in public transit optimization, a bus might get modeled as a capacity, route, and fuel level---all other characteristics are removed from consideration.

\textit{How is it being measured?} Research on optimization often focuses on methods for solving and approximating certain types or groups of optimization problems. Accordingly, much of the attention devoted to optimization isn't concerned with the measurement of particular quantities. Instead, it is assumed that quantities are well-defined and measurable. Therefore, measurement is notably far afield from academic research related to optimization. When optimization is used to guide real-world decision-making, however, measurement becomes a necessary component to understand the impacts and constraints of a decision. Measurement is never perfect; and any measurement technique inevitably introduces \textit{error}. Designers of optimization models must decide what to do about error: for example, they may ignore it, leaving it out of the optimization, or they may use stochastic optimization \cite{heyman2004stochastic, sahinidis2004optimization} to directly model uncertainty.

\textit{Example: \textbf{Transportation}}.
To better understand how measurement considerations play into an optimization model, consider the example of a logistics company that aims to optimize routes for its delivery vehicles. To perform this sort of optimization, the company may want to consider the way that refueling constrains its decision. The resulting optimization may assume that trucks have a certain unchanging fuel efficiency in miles per gallon (MPG) to make it easy to relate route distances to gasoline use. Doing so would rely on a certain kind of measurement (average MPG for a vehicle) to relate two modeling variables (route distance and gas usage), without requiring further measurement about how fuel efficiency varies depending on truck speed, number of traffic lights, fuel grade, price, and other factors. Assuming a static fuel efficiency greatly reduces what must be measured by making a simplifying assumption about how a quantity is measured. 

\subsection{Computing} \label{subsec:compute}

A dominant strand of research on optimization is concerned with computing and computability. Research findings in the field of Operations Research include algorithms to solve optimizations (e.g. \cite{nelder1965simplex, johansson2008subgradient, beck2003mirror}) and methods to approximate optimal values (e.g. \cite{kempe2003maximizing, nikolova2010approximation, kasperski2006approximation}). In some cases, computability is in tension with accurately and comprehensively modeling the state of the world. For example, an objective function may be multi-modal or non-differentiable in practice, but accurately modeling these features would make the optimization computationally difficult to solve. As such, optimization commonly relies on \textit{relaxation} to transform a domain-specific, computationally-intensive optimization into a familiar, solvable type of optimization, ideally one that yields the same or a provably nearby solution. In the process of solving these optimizations, sometimes an optimal solution is still too computationally expensive to attain, so \textit{approximation algorithms} \cite{williamson2011design} are similarly used to find a solution that is nearly-optimal. In this section, we describe these two steps --- \textit{relaxation} and \textit{approximation} --- and aim to excavate their normative assumptions.

\subsubsection*{Relaxations} Relaxations are the transformation of an optimization into another optimization that is easier to solve or work with. The formal definition of the sort of relaxation we refer to in this paper is as follows:

\begin{definition}[Relaxation] \label{def: relax}
    A minimization problem $Q$ is said to be a relaxation of a minimization problem $P$ if the following conditions are met: \begin{enumerate}
        \item $F(P) \subseteq F(Q)$, where $F(x)$  is the feasible decision set defined by the decision and constraints of optimization $x$.
        \item The objective function of optimization $Q$ is less than or equal to that of $p$ for all parameter values in $F(P)$.  \cite{geoffrion1974lagrangean}
    \end{enumerate}
\end{definition}

%\paragraph{Example: \textbf{Integer Programming}} Integer programming problems\footnote{Integer programming problems are a type of mathematical optimization where the solution (decision) can only be integer-valued. For example, in deciding a number of jets to fly between LAX and Laguardia airports, the solution must be an integer. For general introductions see \cite{wolsey2020integer, conforti2014integer}.} may undergo LP-relaxations \cite[p 352]{vanderbei2014integer} so that the solution is easier to compute or approximate.

\subsubsection*{Approximations} Approximations are quantities or methods that are nearly correct. Relaxing an optimization and using the solution as an answer to the original problem (as described above) is one type of approximation. Here we focus specifically on \textit{approximation algorithms} or ways of approximating certain types of optimization problems \cite{williamson2011design, vazirani2001approximation}.

\begin{definition}[Approximation algorithm] \label{def: approximation}
    An $\alpha$-approximation algorithm for an optimization problem is a polynomial-time algorithm that for all instances of the problem produces a solution whose value is within a factor $\alpha$ of the value of an optimal solution \cite[p 14]{williamson2011design}.
\end{definition}

Approximations can happen after an optimization has already been relaxed or fully defined; they do not necessarily rely on expanding the feasible set or changing the objective function as relaxations do. Instead, approximations are often algorithmic approaches that can be incorporated into a computational solver (see Figure \ref{fig:lifecycle}). Using approximations to solve an optimization problem requires making a number of assumptions---for example, it is assumed that a sub-optimal solution with nearly-optimal utility performance is acceptable as a decision outcome. Without formally reporting and considering performance guarantees ($\alpha$ in Definition \ref{def: approximation}), those who apply optimization methods may land on approximate solutions that are far from optimal without knowing it. Such pitfalls are discussed further in Section \ref{subsec:sloppy}.

Relaxations and approximations suggest a trade-off between at least two desiderata: reducing computational complexity and maintaining performance (e.g., $\alpha$). Of course, modelers are juggling a number of other potential goals as well, including consistency \cite{evers2009regrouping, fedrizzi2007incomplete}, robustness \cite{beyer2007robust, gabrel2014recent, ben2002robust, bertsimas2011theory}, and correctness \cite{samet1978proving, fluckiger2017correctness, d2015correctness}. Trade-offs between goals abound in optimization, and have been discussed especially in machine learning contexts \cite{belkin2019reconciling, zhang2019theoretically, kleinberg2016inherent, cooper2021emergent}. These trade-offs may or may not receive explicit consideration from model designers. However, whether or not the designer has explicitly taken these values into consideration or weighed between them, the underlying values and normative commitments are reflected in an optimized decision. 

\subsection{Application} \label{subsec:apply}

Optimization research tends to categorize and solve problems based on particular groupings or structures of problems. Often, solution algorithms are found through a process of typifying the the objective function and constraints and demonstrating solutions that work on certain general categories of problems (e.g., convex problems \cite{boyd2004convex}). Solutions, approximations and relaxations are then developed for these various already-abstract problems without considering domain-specific contexts or scenarios.

Our characterization of optimization research as abstracted from real-world scenarios is not intended as an indictment of the research but instead provides lessons for how optimization might be safely and ethically applied in real-world domains. When applying optimization, it is essential to consider whether the application is reasonable in the real, non-abstract context, or whether it is is, for example, far-fetched, impossible, or unethical. Especially when objectives are contested, numerous, complex or conflicting, researchers and practitioners sometimes find that the right choice is refusal to adopt or use a technological tool \cite{simpson2007ethnographic, zajko2022artificial}.

When optimization is applied in real-world settings, decision-makers necessarily make assumptions about \textit{applicability} to conclude that an optimal solution is the right course of action. Assumptions are made about both the \textit{impact} of the optimization\bldelete{ (see Figure \ref{fig:lifecycle})} and the \textit{relation} between the decision and other decisions. Often, even though individual decisions are said to be optimized, the process of optimization requires tweaking, iteration, and repeated use over multiple decisions.\footnote{Failing to model the decision as dynamic has been noted by \citet{selbst2019fairness} as a potential vulnerability for decision-making in socio-technical systems. The authors refer to this issue as the  \textit{ripple effect trap}.} The dynamics arising from  applicability assumptions may generate forms of instability: system oscillations \cite{zhu2018optimization}, runaway feedback effects \cite{ensign2018runaway, lum2016predict}, amplification, or domain drift \cite{tomani2021post} over time.

\bldelete{\textit{Example: \textbf{Electric scooters}} Optimization plays a significant role in small-vehicle logistics and operations \cite{baouche2014efficient, sandoval2021data, zhu2021optimal} Electric e-scooter fleet companies decide where to deploy vehicles each morning and typically make their allocation decision according to an optimization. This optimization may be designed to take into account the location of vehicles and predicted demand the next day, but may choose (not) to consider the impact of day 1’s optimization on day 2’s fleet. Their decision is actually one of a set of sequential decision and the domain is therefore \textit{dynamic} in nature.}

==> sections/conclusion.tex <==
%\section{Conclusion} \label{sec:conclusion}

==> sections/introduction.tex <==
\section{Introduction} \label{sec:intro}

Mathematical optimization\footnote{For the formal definition used throughout this paper, see Appendix \ref{app:opt}.} is a way to relate a set of potential decisions to a specific goal and use this relationship to identify the best-performing decision. It is a paradigm used in industry and government and aids in developing a variety of computing tools including machine learning (ML) models. Optimization’s widespread use and applicability is enabled, in part, by its level of abstraction. By representing real decisions as a set of \textit{decision variable(s)}, \textit{objective(s)}, and \textit{constraint(s)}, optimization methods identify solutions that maximize the objective while meeting the relevant constraints. 

However, optimization does not necessarily imbue a decision with legitimacy or ethical justification. Because such a broad set of parameters and functions are left to be specified, an optimization can be designed to serve subjective or parochial interests, out of step with social welfare. For example, when a social media advertiser uses optimization to target ads in a way that maximizes user engagement, it may not be the case that the so-called `optimized' decision is one that is best for society. 

This paper aims to highlight optimization’s normative choices and assumptions. In Section \ref{sec:lifecycle}, we describe the \textit{life cycle} of an optimization, particularly as it is used in operational decision-making, machine learning, and research. Our treatment of the life cycle or pipeline associated with applied optimization is intended to be reminiscent of existing characterizations of the \textit{machine learning life-cycle} which have proven useful for end-to-end analysis \cite{suresh2021framework,hutchinson2021towards,garcia2018context,souza2019provenance,cao2021toward,lauferend}. We then focus on the various choices and assumptions inherent in the optimization life cycle, which we categorize into the following components: modeling, measurement, computing, and application. In Section \ref{sec:neglect}, we identify six emergent issues that may be neglected: \textit{1) misspecified values, 2) inaccurate decision boundaries, 3) failing to account for multiple agents, 4) label mismeasurement, 5) faulty use of relaxation and approximation, and 6) treating optimization as a justification for action.} Finally, Section \ref{sec:programme} articulates suggestions and directions for research on optimization and its normative implications.


==> sections/pipeline.tex <==
\section{The Optimization Life Cycle}\label{sec:lifecycle}

Examining the assumptions and choices laden in an optimization requires thinking about optimization as a sociotechnical process. In this section, we describe the typical steps in the \textit{life cycle} (or \textit{pipeline}) associated with applying optimization in real-world settings. An equivalent life cycle for ML systems has been developed and widely used (see e.g. \cite{souza2019provenance, garcia2018context}) including as a framework for evaluating normative assumptions and potential harms  \cite{suresh2021framework, lee2021risk, ashmore2021assuring, cao2021toward,lauferend}. We propose an analogous pipeline that describes an archetypal use of optimization. Equipped with such a pipeline, we will systematically analyze optimization's component choices and assumptions to unearth normative commitments. A visual representation of the optimization life cycle is provided in Figure \ref{fig:lifecycle}.

To characterize the use of optimization from its inception (measurement and modeling) to its execution (solving and applying), it is important to note that optimization can look very different depending on the context. Thus, we'll start by discussing some domains where optimization is commonly applied. Then, we'll discuss the component steps involved in a typical optimization process.

\subsection*{Common Contexts}

Here we discuss three common application domains for optimization: operational decision-making, machine learning, and scientific research.

\subsubsection*{Operational Decision-Making} \label{subsec:operational}

Optimization is perhaps best understood as a method to approach complex logistical decisions. These decisions aim for operational efficiency for large-scale industrial or institutional endeavors with significant complexity. Canonical examples cited in introductory optimization courses include signal processing and networked communication \cite{luo2003applications, neely2010stochastic}, portfolio optimization in financial mathematics \cite{black1992global, perold1984large, cvitanic1992convex, jorion1992portfolio}, and transportation \cite{bielli2002genetic, mandl1980evaluation, osorio2013simulation}. 

For examples of high-impact optimization problems applied to decision-making, one can simply look to the history of linear programming.\footnote{Linear programming is one particular type of optimization where the constraints are a set of linear inequalities and the objective is a linear equation. In the early twentieth century, Optimization
was more commonly known as ``mathematical programming,” where the word \textit{programming} referred to decision-making rather than computer programs (computers had yet to be invented).} LP problems gained prominence in both the US and USSR during the Second World War, where mathematicians and economists in both countries began considering how to devise optimal large-scale policies with limited budgets --- these policies ranged from wood production to air force allocation \cite{singhbrief}.


\subsubsection*{Machine Learning} \label{subsec:ml}

Optimization and machine learning are intimately related and machine learning often relies on optimization. The algorithms used to train a ML model may use a formal notion of \textit{loss}---for example, prediction error---in the training process. Fitting parameters to \textit{minimize} this loss can be written as an optimization problem.

For example, a univariate linear regression using ordinary least squares (OLS) finds a line to fit the data. Of all possible lines which could be used to describe the relationship in the data, the `line of best fit’ according to OLS is the line which minimizes the sum of squared errors between the predicted values and the observed data. This task can be written as an optimization problem, where the decision variables are the slope $m$ and the intercept $b$ of the line. The feasible set is all real numbers (the problem is unconstrained beyond $m,b \in \mathbb{R}^2$). And the objective is to minimize loss, namely the sum of squared errors.

For more complex models using high-dimensional datasets, the optimizations become more tedious to write out but the idea is the same: Some notion of loss is defined so that the model fit will resemble the observed training data, and defining the model involves solving an optimization to minimize loss.

Although we predominantly draw from examples in logistical decision-making and management science, we believe that this paper’s framework yields useful insights about optimization’s role in the machine learning pipeline. For example, defining loss is a choice with particular priorities and commitments. Sometimes, this decision is made simply by choosing a loss metric which is computationally easy to work with. Another example of this paper’s usefulness in scrutinizing ML is in assumptions about decisions and decision boundaries: Often, ML predictions are translated into decisions without considering the impacts, social implications, or feedback effects associated with the particular decision.\bldelete{ This phenomenon is written about more extensively in \citet{selbst2019fairness}'s discussion of \textit{ripple effects} in socio-technical systems.}

\subsubsection*{Scientific Research} \label{subsec:sci}

Optimization crops up in a number of disciplines outside of operations research, math and statistics. Where optimization is applied to scientific research, it may guide design decisions for building scientific instruments \cite{chen2005design, niu2014design, zheng2012design} or in the discovery of new drugs to test \cite{ou2012computational, prada2016application, caldwell2001new, de2020silico, copeland2013evaluation}. These are examples of \textit{operational} uses, similar to those described above.

Another use for optimization in research is as a descriptive tool. For example, researchers employ agent-based models to understand complex processes, and optimization often plays a role in simulating how modeled agents behave. The use of optimization in simulation or theoretical models is distinct because it is used to describe the behavior of an agent. The optimization is used to draw descriptive conclusions that do not necessarily guide real-world decisions. Optimization in this sense \textit{describes} rather than \textit{dictates}. For example, in game theory’s applications to economics \cite{sohrabi2020survey, aghassi2006robust,curiel2013cooperative, scutari2010convex} and biology \cite{hammerstein1994game, dugatkin2000game, grupen2020low, leboucher2018enhanced}, optimization is used to model agent decisions and strategies. Pinpointing assumptions and normative imperatives within these optimizations may be useful---they may reveal values and priorities held by researchers, or assumptions made about economic subjects. However, because these optimizations are not used to justify a particular `optimized' decision, we do not draw examples from these domains and consider them to be out of scope.



\begin{figure*}
    \begin{center}
    \includegraphics[width = \textwidth]{figures/Latest Optimization Lifecycle 5-11.pdf}
    \end{center}
    \caption{The optimization life cycle, beginning with measurement and data generation and ending with operational decision-making and real-world impact.}
    \label{fig:lifecycle}
    
\end{figure*}



==> sections/problems-new.tex <==
\section{Emergent Problems and Neglect}\label{sec:neglect}

The optimization paradigm requires a number of choices, simplifications, and assumptions, as demonstrated in Section \ref{sec:assumptions}. These choices can contain particular commitments and serve particular interests. A company's goals, priorities, values, norms, and conventions can influence the considerations that end up in an optimization model. As such, `optimal' decision-making in one company or sector means something very particular and context-dependent. A decision described as `optimal' or `optimized' is not, necessarily, a virtuous decision.

Our contention is that optimization is a powerful tool; its use is not ethically neutral simply because it is quantitative and scientific.\footnote{Relatedly, applications of \textit{mechanism design} have been referred to as `technologies of depoliticization' \cite{hitzig2020normative}. See also \citet{viljoen2021design}, \citet{hitzig2019technological}, and \citet{finocchiaro2021bridging} on mechanism design’s normative dimensions. Mechanism design can be described as a type of optimization and, similarly, can invoke objectivity or impartiality.} Optimization can be used for a number of desirable or undesirable ends, and its application can lead to emergent issues and downstream consequences. We do not argue that optimization’s constituent choices and assumptions are inevitably problematic. Instead, we use the process (or life cycle) of optimization to identify ethical pitfalls, harms, and wrongs that can emerge. 

\subsubsection*{When are these problems `neglected'?} To neglect is to \textit{fail to care for properly}. The worry with optimization is that it can appear to be objective and exhaustive. Optimization is a systematic paradigm used to approach decisions, constraints, and goals, however, its use does not guarantee that all relevant decisions, constraints, goals, interests, values, and other considerations have been adequately weighed. As we describe in this section, there are several cases where optimizations do not properly account for particular harms or values. When an optimization does not take proper consideration of ethically relevant interests or consequences, these interests or consequences may be described as \textit{neglected}.

To be sure, some emergent problems and downstream consequences are unknown and unforeseeable. For example, consequences that are far enough in the future, or that arise from apparent anomalies, may be exceedingly difficult to predict and account for in a decision calculation. These harms and wrongs are difficult to attribute to a lack of care. But, by observing and documenting known problems and failure modes, these cases can inform standards of care and accountability mechanisms.

This section puts forward six emergent issues that can be overlooked when optimization is used to justify or derive a decision. These issues arise at various steps throughout the optimization life cycle. Where relevant, we provide examples and offer suggestions.

\begin{table*}[htp]
\caption{Breakdown of categories of assumption, neglected problems, and emergent issues in the optimization life cycle.}
\label{table:summary}
\footnotesize
\begin{center}
\begin{tabular}{l l l}
\toprule
% headers
\textbf{Life Cycle Steps} &   \textbf{Emergent Problems}   &   \textbf{Particular Issues}   \\
\midrule
% [<number>] controls vertical text placement
\multirow{7}[7]{*}{Modeling (\ref{subsec:model})}   

   &   \multirow{3}[3]{*}{Misspecifying Values (\ref{subsec:misspecifyingvalues})} & Omitting Values (\ref{subsubsec:omittingvalues}) \\
   
   \cmidrule{3-3}
   
   & & Mistakenly Modeling a Value as a Constraint (\ref{subsubsec:mistakenlymodelingconstraint}) \\
   
   \cmidrule{3-3}
   
   & & Mistakenly Modeling a Value as an Objective (\ref{subsubsec:mistakenlymodelingobjective})\\

   \cmidrule{2-3}
   
   & \multirow{2}[2]{*}{Problematic Decision Boundaries (\ref{subsec:imprecisedecisionboundaries})} &
    % divided row
            Faulty Modularity Assumptions (\ref{subsubsec:faultymodularity})  \\
    \cmidrule{3-3}
    % divided row -- second line
    &  & Feedback Loops (\ref{subsubsec:feedbackloops}) \\
        
% third super row
\cmidrule{2-3}

   &   \multirow{2}[2]{*}{Neglecting to Consider Multiple Agents  (\ref{subsec:neglectingtoconsidermultipleagents})} & Objective Reflects Narrow Interests (\ref{subsubsec:objectiverepresentsnarrowinterests})  \\
   
   \cmidrule{3-3}
   
   & & Decision Model Formalizes Notions of Control (\ref{subsubsec:decisionmodelformalizes})\\

   \midrule
% [<number>] controls vertical text placement
\multirow{2}[2]{*}{Measurement (\ref{subsec:measure})}   &   \multirow{2}[2]{*}{Label Mismeasurement (\ref{subsec:labelmismeasurement})} &
    % divided row -- first line; this is busted but at least it works
            {Imprecise Labels (\ref{subsubsec:impreciselabels})}      \\
    \cmidrule{3-3}
    % divided row -- second line
    & & Biased Labels (\ref{subsubsec:biasedlabels}) \\
% second super-row

\midrule
% [<number>] controls vertical text placement
\multirow{2}[2]{*}{Computing (\ref{subsec:compute})}   &   \multirow{2}[2]{*}{Faulty Solution Steps (\ref{subsec:sloppy})} & Faulty Use of Relaxations (\ref{subsubsec:sloppyrelaxations})
    % divided row -- first line; this is busted but at least it works
                \\
    \cmidrule{3-3}
    % divided row -- second line
    & & Faulty Use of Approximation Algorithms (\ref{subsubsec:sloppyapproximation})  \\

% fourth super-row
\midrule
% [<number>] controls vertical text placement
\multirow{2}[2]{*}{Application (\ref{subsec:apply})}   &   \multirow{2}[2]{*}{Using ``Optimal'' as Justification (\ref{subsec:usingoptimalasjustification})} & Justificatory Language (\ref{subsubsec:language})\\
    \cmidrule{3-3}
    % divided row -- second line
    & & Reverse Engineering/Retrofitting (\ref{subsubsec:formal})  
            \\
   
\bottomrule
\end{tabular}
\end{center}
\end{table*}


\subsection{Misspecifying Values} \label{subsec:misspecifyingvalues}

Optimization requires formally specifying at least one decision and at least one notion of measurable value or utility. The values laden in optimization are made most apparent by the existence of an objective function, which formalizes a goal that the decision-maker is assumed to wish to maximize. Aligning values with optimization objectives of significant interest \cite{hadfield2016cooperative, milli2021optimizing}. But values play into other components of a model besides the objective. For instance, models often include constraints motivated by ethical norms or values like fairness.

Here, we discuss the issues that arise when a model is misspecified in such a way that values are not given rightful consideration. We identify two mechanisms that result in misspecified values: 1) leaving values out of an optimization completely and 2) mistreating or mismodeling values within an optimization. In discussing the latter type of misspecification, we consider instances where values are wrongfully incorporated as optimization constraints (instead of objectives), or wrongfully incorporated as objectives (instead of constraints). 

\subsubsection{Omitting Values} \label{subsubsec:omittingvalues}

Omitting values from an optimization problem can be either careless or deliberate. A careless omission of values arises when the humans designing and executing an optimization fail to properly consider the ramifications of their modeling or measurement assumptions. For example, a company that makes custom shirts might decide where to source their textiles. An optimization problem that minimizes the cost of textiles might suggest changing which factory they contract with. However, it could be that the new factory has dangerous working conditions or otherwise harsh and unethical labor policies. If the optimization designer was unaware of this distinction, the omission of labor considerations from the decision would be \textit{careless}; if they were aware, it would be \textit{deliberate} and malicious.

Scrutinizing which values and implications are included or excluded from an optimization provides important information for attributing harms and establishing \textit{accountability}, but one cannot differentiate negligent and deliberate omissions from the optimization model alone --- further contextual evidence is needed to qualify the human decisions behind an optimization model. In the case that a value is omitted from an optimization on purpose, agents may use the optimization's output as \textit{justification} for a certain decision. We turn back to this idea in Section \ref{subsec:just}.

\subsubsection{Mistakenly Modeling a Value as a Constraint} \label{subsubsec:mistakenlymodelingconstraint}

Often a constraint is added to a model which is based on a moral imperative: A new housing development in a lower-income neighborhood may be required to reserve a certain number of units as rent-stabilized, low- or middle-income housing, leading developers to treat this requirement as a constraint on building a profitable new development. When companies boycott sales in foreign areas to voice dissatisfaction with states’ political decisions, their resulting business strategy is constrained by their stance; even if their supposed goal is profit and expansion. When somebody decides to go on a diet and cut out added sugars, similarly, they approach their food decisions with constraints because resetting the objective may be more difficult to hard-wire.

These values are assumed to be categorical, rules-based, and violating them becomes fully infeasible when they are incorporated as a constraint. Values such as \textbf{\textit{fairness}} are assumed to be constraints, even though concepts such as \textbf{\textit{equity}} may readily be considered utilities to be maximized. Though constraints play an important role in determining the feasible set of decisions available to a decision-maker, they can also be weak in guiding values judgments: As long as a decision is feasible, constraints play no role in preferring one decision over another. So, within the feasible set, a constraint has no bearing on what option gets chosen. What's more, non-negligible constraints that are added to an optimization tend to yield solutions that lie on these constraints: \textbf{\textit{solutions tend to `bump up against' constraints.}} In practice, this can mean that `optimal' solutions do the \textit{bare minimum} at meeting some values-driven imperative.

\textit{Example: \textbf{Access}}. Consider a city which has two potential ways of providing transportation to its people. One option is to allow private industry to provide transportation through contracts with the city. In this case, providers might reach decisions with the city that constrain their behavior, for instance that they must provide a certain level of access to low-income neighborhoods. At the end of the day, however, their objective is to \textit{maximize profit} subject to \textit{legal constraints}.  An alternative option is to treat transportation as a public service, where a single entity with a budget is tasked with providing transportation. In this public approach, an agency might aim to \textit{maximize access} subject to \textit{budgetary constraints}. These two approaches to optimization logic encode the same values (access and budgetary responsibility) but do so in ways that can lead to vastly different levels of access across communities.

\subsubsection{Mistakenly Modeling a Value as an Objective} \label{subsubsec:mistakenlymodelingobjective}

An objective function defines utility as a quantifiable and measurable function of the relevant decision $x$. This way, for any particular decision value $x_i$, the utility of that decision can be directly compared (via a quantitative scale) to an alternative decision $x_j$. Defining the objective lends itself well to \textit{ends-based} or \textit{utilitarian} frameworks\footnote{Quantification and prediction are key facets of utilitarianism, which as an ethical project aims to maximize utility. A relevant paper which discuss the theme of operationalization and utilitarianism is \cite{zame2007can}.} which treat value as quantifiable and to some extent predictable \cite{sinnott2003consequentialism}.\footnote{Some forms of consequentialism acknowledge that ends are inherently unpredictable. Rule consequentialism \cite{hooker1990rule}, for example, is an ethical theory which uses an ends-based framework to justify heuristic rules, since ends cannot easily be predicted by humans. However, even these theories assume that standards can be derived by their expected (predicted) outcomes, even if predictions always have significant error.}  In fact, an optimization model presumes to model the relationship between a decision and its utility outcome---in non-stochastic optimizations, this relationship is presumed to be fully known and defined, whereas stochastic optimization models randomness explicitly \cite{sahinidis2004optimization}. Sometimes, values are treated as objectives when they ought to be modeled elsewhere in an optimization. These instances tend to involve misplaced incentives---a company is incentivized to maximize profit, even if they should really be incorporating other notions of utility in their optimization. 

\textit{Example: \textbf{Safety}}. Car companies communicate that they aim to build the safest cars. In reality, these companies have many goals including engine efficiency, speed, comfort, and profit. If safety were truly the utmost objective, a car would not move: staying parked is the safest state for a car. Of course, the functionality of a car requires that safety is not always modeled as a \textit{sole} objective (even if such an objective is communicated in advertisements). More realistically, many car companies' safety considerations are treated as \textit{constraints}.\bldelete{ A similar case can be made for telecommunication companies’ relationship to \textit{\textbf{privacy}}---the devices and networks created functionally create ramifications for privacy; and optimizing for privacy alone would be futile.}

\subsection{Problematic Decision Boundaries} \label{subsec:imprecisedecisionboundaries}

A first step in specifying an optimization model is defining and constraining the \textit{decision variable}. Specifying which variables are freely tunable and which values are feasible lays the roadmap for solving the optimization. Doing so dictates the set of potential outcomes, how the problem may be solved, and, perhaps most importantly, what factors are within vs outside the control of the decision-maker.

Specifying the decision involves assumptions about \textit{who makes the decision} as well as \textit{what power they have over the state of the world}. Making such assumptions risks glossing over the mechanism through which a decision-maker enacts change, and a variety of requisite or related decisions that may be involved. The remainder of this section is devoted to 1) neglectful decision boundaries for synchronous decisions (which arise because of \textit{faulty modularity assumptions}) and 2) neglectful decision boundaries for asynchronous decisions (which can lead to \textit{feedback loops}).

\subsubsection{Faulty Modularity Assumptions} \label{subsubsec:faultymodularity}

It can be simpler or convenient to treat problems as separate optimizations when the number of decisions is too vast. The optimization paradigm makes it very easy to divide and conquer by treating the solution of one optimization as an (unchanging) parameter in a second problem.

Imprecise decision boundaries, including incorrect assumptions about modularity, lead to narrow optimizations that may not serve the broader function of a system or a society. Divide-and-conquer optimization strategies, with incorrect modularity assumptions, can have unanticipated normative and political implications. For example, \citet[p 245]{mulligan2020concept} use the example of access control to illustrate this point: although tech companies can justify switching from passwords to fingerprints to face ID by saying each new technology more \textit{optimally} performs the specified function of access control, such changes have notable political implications; for instance each successive handoff might be said to curtail user control and diminish transparency.\footnote{See also \citet{goldenfein2020through}.} Improvements or optimizations directed at sub-functions of a larger system should consider broader societal implications and interests. Otherwise, optimization alone does not justify exchanging or updating a technological sub-component.

\textit{Example: \textbf{Transit}}. Consider a metropolitan transit authority faced with the following decisions: given budget and staff constraints, how much to charge in tolls and whether (or which) lanes should be restricted to high-occupancy vehicles during peak travel times. In actuality, these decisions are not independent: how much a highway charges in tolls will impact the number of cars on the road by inducing demand, which in turn is important for evaluating to what extent high-occupancy vehicle lanes will improve overall traffic throughput. Similarly, how many lanes will be restricted---or the window of time during which the restriction is enforced, or how costly the fine---will constrain how many people may commit to carpooling and significantly affect budget and revenue considerations for the toll decision. These choices could be treated in isolation: first, decide how many restricted lanes would serve the carpooling population, and then (conditional on a set number of lanes) decide what to charge in tolls. But to do so would ignore the fundamentally interdependent nature of the decision, and may generate spillover effects that the simplistic model does not account for.

\subsubsection{Feedback Loops} \label{subsubsec:feedbackloops}

Optimizations may arise in a repeated fashion where it is unreasonable to assume each sequential decision is independent. For the same reason numerous synchronous decisions may be haphazardly split into separate optimizations (discussed in Section \ref{subsubsec:faultymodularity}), modelers may unreasonably assume sequential decisions are independent.

The phenomenon of feedback in optimization is represented in Figure \ref{fig:lifecycle}'s depiction of the entire optimization life cycle as a loop. Optimizations can be used repeatedly, even if the formal operational strategy does not account for one optimization’s impact on the next. Similar feedback loops have been observed in statistical systems that do not necessarily involve optimization --- in domains ranging from mechanisms and acoustics to economic inequality, the concept of feedback and path-dependence explains patterns where compounding or overlapping impacts from multiple sequential events lead to unanticipated or chaotic events. In the context of fairness for socio-technical systems, \citet[p 62]{selbst2019fairness} described this phenomenon (and corresponding neglect on behalf of designers) as the \textit{ripple effect trap}.

In the case of optimization, it may be that an optimal decision in one instance is sub-optimal or actively harmful when repeated sequentially over time. A common example of this difference comes from bad modeling set-up or incorrect assumptions can lead an agent to so-called `greedy' policies where they always exploit known reward, or always explore new and high-risk options (see e.g. \cite{bubeck2009pure}). \textit{Multi-armed bandit} problems \cite{bubeck2012regret, vermorel2005multi, lu2010contextual} reflect this dynamic: knowing that an agent has many decisions that can be made in sequence, it may be optimal to explore new unknown choices. Agents with only one decision, however, may instead opt to exploit their known option with the highest value.
 
\textit{Example: \textbf{Predictive Policing}}. The tendency to \textit{exploit} when sequential optimizations are treated as individual decisions has been shown to cause harmful disparities in treatment. To illustrate this point, consider the example of PredPol (now re-branded as Geolitica), a commercial predictive policing software that used historical data to statistically train optimal\footnote{The predictive algorithm developed by PredPol used expectation-maximization techniques developed in \cite{mohler2014marked}, as noted in \cite{mohler2015randomized} and \cite{ensign2018runaway}.} policing recommendations \cite{mohler2015randomized}. The software was accused of formalizing and entrenching historical biases \cite{lum2016predict, isaac2017hope, silva2018algorithms}. Theoretical models of sequential predictive decisions provided an explanation for these emergent biases: Predictions made as single-shot optimizations can introduce \textit{runaway feedback effects} when applied sequentially over time, since predictive algorithms direct police to neighborhoods where crime was historically observed \cite{ensign2018runaway, laufer2020compounding}.


\subsection{Neglecting to Consider Multiple Agents} \label{subsec:neglectingtoconsidermultipleagents}

A notable feature of optimization is its strict delineation between decision variables and other (non-decision) variables: Certain parameters are considered to be in the control of the decision-making agent, and other parameters are exogenous and outside the direct control of the agent. This approach makes it convenient to divide optimizations into individual, simple decisions as described in Section \ref{subsec:imprecisedecisionboundaries}. The approach also lends itself to treating decisions as belonging to a \textit{singular agent}. Even though optimizations are commonly used by institutional bodies and passed between numerous stakeholders ranging from analysts to engineers to executives, these optimizations may not consider that the various constituents of an organization are distinct decision-makers themselves. In this section, we consider how optimization problems may neglect to properly consider the agency of multiple decision-makers, and how such neglects can be avoided or identified. When multiple agents are not taken into consideration, optimizations may only serve the interests of a few people, and additionally may codify or formalize particular structures of management and control. In this section, we consider each of these emergent issues. 

\subsubsection{Objective Represents Narrow Interests} \label{subsubsec:objectiverepresentsnarrowinterests} Optimization is used to make logistical decisions that can impact many people, both inside and outside the decision-making apparatus. For a given optimization, the relative importance of different agents’ utility can be defined in the objective function. When an objective omits or de-values harmful impacts on certain populations, the resulting ``optimal'' decision can be ethically wrongful.

When an objective reflects only certain interests in an organization, the optimal decision might justify exploitative working conditions. Take the toy example of a board of directors deciding how to use a certain amount in earnings. Without union representation on the board, they might decide that their utmost priority is to keep investors happy and therefore pay dividends. With union representation, however, they might adjust their priorities and devote more earnings to employee compensation. The choice of \textit{goal} or \textit{objective} is highly dependent on the organizational structure.\footnote{We refer readers to \citet{kasy2021fairness}, which puts forward a formal notion of \textit{power} as it relates to designing the objective function.}

\textit{Example: \textbf{Technology Adoption}}. When financial mathematicians began to suggest that optimization could improve portfolio diversification schemes, firms were slow to adopt these schemes. In one academic paper devoted to the reasons why firms did not adopt these measures, a reason for the resistance was the social and political structure of the firm: ``Probably the single most important reason why many financial institutions don't use portfolio optimizers is \textbf{political}. This is because the effective use of an optimizer mandates significant changes in the structure of the organization and the management of the investment process'' \cite[p 32]{michaud1989markowitz}. Firm managers did not want to cede decision-making power to quantitative analysts, suggesting internal organizational social structure influences the use of optimization. 

The ``narrow interests'' described so far concern internal social structures in a decision-making apparatus. But problems of narrowly defined goals can also have massive impacts on people external to the decision who have little or no relation to the particular company or institutional body's decision. The notion of \textit{externalities} \cite{ayres1969production, baumol1972taxation, cornes1996theory} (see also \cite{coase2013problem}) helps to describe how unaccounted-for impacts can affect people who might face barriers entering into contracts or fending off negative consequences. People downstream from a river might be negatively impacted by factory pollution and may not even know it. These effects can be the result of negligent or malicious tweaks to an objective function. They highlight the importance of critically evaluating optimizations and their stated goals.

\subsubsection{Decision Model Formalizes Notions of Control} \label{subsubsec:decisionmodelformalizes} Moving beyond how the objective is defined, the \textit{decision variables} in an optimization are an important indicator for what an agent has control over. In formalizing exactly what decision is assumed to be under the control of an agent or organization, an optimization can codify existing social structures.

\textit{Example: \textbf{Workforce Optimization}}. Industries are fiercely competitive over employee talent, and retaining employees has become an important priority for companies. So-called `workforce optimization' \cite{roy2019enabling, naveh2007workforce, altner2018two} or `staff planning problems' \cite{anderson2001nonstationary, balachandran1982interactive, abernathy1973three} devise strategies to allocate, promote and pay workers in order to maximize retention and efficiency while minimizing employer costs. Such models make assumptions about a particular type of employee/employer relationship, for example that employees are contractors whose time can be allocated freely; or that layoff recommendations can come from performance metrics rather than human judgments. The clearest examples of decision models formalizing or implicating systems of control are warehouse management and logistics studies that create staffing tools for warehouse managers that balance worker discomfort, worker risk, and efficiency \cite{wruck2017risk, larco2017managing}.\footnote{These tools are further discussed in \cite{gong2011review, de2017warehouse}.}


\subsection{Label Mismeasurement} \label{subsec:labelmismeasurement}

Issues in the choice of labels and measurements can lead to undesirable outcomes in the application of optimization. Inaccurate labels exhibit errors whereby there is some characteristic distance between a measurement and a true value. In this section, we discuss two types of label mismeasurement which lead to inaccuracy: imprecise labels and biased labels. These mismeasurements can either be a \textit{conceptual error}, whereby proxies or incorrect labels are used instead of a true underlying value, or a \textit{measurement error}, whereby instruments or empirical methods do not work as expected. Accuracy is comprised of both precision and the absence of bias in measurement--below, we briefly discuss label mismeasurement in terms of these two components.

\subsubsection{Imprecise Labels} \label{subsubsec:impreciselabels} 

Imprecise labels are labels with a high degree of uncertainty or low level of significance. A measurement can be precise and inaccurate if it tends to detect values to a certain level of precision, but those values are consistently biased. A measurement is imprecise when its measurement exhibits significant random error. 

\textit{Example: \textbf{Portfolio Optimization}}. After Harry Markowitz put forward a method to optimally diversify portfolios in such a way that maximizes expected return \cite{markowitz1991foundations, markowitz2000mean}, practitioners who tried applying the method found that it under-performed human decisions and even simple equal-weighting methods \cite{Jobson70}. In an article aptly titled ``The Markowitz Optimization Enigma: Is `Optimized' Optimal?'' \cite{michaud1989markowitz} it was shown that, systematically, assets with the highest measurement error were also those that had the highest expected return. \citet[p 68]{jorion1992portfolio} described the issue: ``A major drawback with the classical implementation of mean-variance analysis is that it completely ignores the effect of measurement error on optimal portfolio allocations ... optimization systematically overweights the assets with the highest estimation errors, hence overstates the true efficiency of the optimal portfolio.''


\subsubsection{Biased Labels} \label{subsubsec:biasedlabels}

Biased labels are consistently inaccurate in a way that predictably and systematically leads to different outcomes for different subjects of an optimization.

\textit{Example: \textbf{Medical Risk Assessment}}. \citet{obermeyer2019dissecting} study a risk prediction algorithm that is used on 200 million Americans annually to optimally distribute health services. The objective function of the risk assessment algorithm trained the algorithm to predict future health \textit{costs} rather than health \textit{needs}, and due to a historical gap in access across race, the risk scores systematically recommended fewer Black patients receive medical resources. Notably, the paper invokes the algorithm's \textit{objective function} in framing its inquiry into the mechanism of bias: ``An unusual aspect of our dataset is that we observe the algorithm's inputs and outputs as well as its objective function, providing us a unique window into the mechanisms by which bias arises'' \cite[p 3]{obermeyer2019dissecting}.


\subsection{Faulty Solution Steps} \label{subsec:sloppy}

The steps involved in solving an optimization problem, from relaxations to iterative algorithmic solutions, involve assumptions and simplifications that ought to be dealt with carefully and notated precisely. In this section, we discuss two types of neglect in the steps involved with solving optimizations: \textit{faulty use of relaxations} and \textit{faulty use of approximation algorithms}. Our goal in this section is not to critique optimization research, which tends to precisely and clearly characterize the use of approximations, nor to critique all applications of optimization. More often, these areas of neglect can occur in private settings which emphasize speed and minimum viability \cite{ries2009minimum, moogk2012minimum} in product development.

\subsubsection{Faulty Use of Relaxations} \label{subsubsec:sloppyrelaxations}

When a relaxation is used for ease of computation or measurement, it can significantly change the optimization's feasible set and objective function.  As such, it is important to detail when relaxations are being used, and what assumptions are made in the process. When a problem is relaxed, its fundamental structure has changed. The solution set might be much bigger, or smaller, than the true optimization problem, for example. As such, calling a solution to a relaxed problem `optimal' may be misleading without appropriately caveating. When relaxations are purposefully concealed and a solution is described as \textit{optimal}, such a practice is \textit{faulty}. It postures as \textit{legitimate} on false pretenses, even when its recommended choice could be misguided or non-optimal.

\subsubsection{Faulty Use of Approximation Algorithms} \label{subsubsec:sloppyapproximation}

It is common for operations researchers, mathematicians, and computer scientists to focus on a particular category of problem, come up with a way of approximating the solution, and prove that the approximate solution is within a certain error bound compared to the true solution. In optimization, maximization (minimization) problems are approximated with answers that perform below (above) the true optimal, in which case lower (upper) bounds are given. Approximations are applied haphazardly when these guaranteed bounds are not given, and the performance guarantee or bound is not specified. Approximation algorithms are also applied sloppily if they are derived for a certain \textit{type} of problem (e.g., convex) and are applied on a different type of problem (e.g., non-convex). Such a behavior can be \textit{faulty} when performance is purposefully over-stated, or uncertainty is concealed.

\subsection{Using “Optimal” as Justification} \label{subsec:usingoptimalasjustification} \label{subsec:just}


The final problem identified in this paper arises when people assume that an \textit{optimal decision} is an \textit{ethically justified decision}. As optimization has entered common parlance, it is used to describe a variety of behaviors and strategies that aim to achieve a variety of ends. Optimization is sometimes invoked without specifying a particular decision or objective---an optimal workforce strategy or an optimal economic policy lack the kind of specificity that is required to understand if a particular strategy is morally or politically desirable. In this section, we discuss the justificatory use of optimization. Particular mechanisms by which optimization can be used to justify action are apparent in language (e.g., when a decision-makers calls their decision \textit{optimal} without further context) and in cases where an optimization problem is retrofit to a decision that has already been made.

\subsubsection{Implicit Subject-Object Relationship} \label{subsubsec:language}

The use of the verb ``optimize,'' when used in the sense we discuss in this paper, implies that there is a \textit{decision} and a \textit{goal}. Sometimes, when people use the word without specifying one of these constitutive components, the context can clarify: ``optimize draft picks" might specify the decision and imply the goal, for example. When the decision and goal are indeterminate and a quantity is claimed to be \textit{optimal}, however, we argue that this description is a category error and its use is a primary suspect for the sort of neglect we are describing. Especially in high-stakes settings, where the goals of a certain decision might be contested, such as admissions, sentencing, and urban policy, using the word \textit{optimal} to describe a particular decision may be a faulty justification or optic maneuver.

\subsubsection{Reverse Engineering} \label{subsubsec:formal}
Beyond the \textit{linguistic} use of optimization to justify behavior, we make a slightly stronger claim: even if an optimization model is defined and solved indicating that a particular decision is optimal, such a process does not morally justify making that decision.  This point can be demonstrated by considering two optimizations, nearly identical, except one switches ``minimize" for ``maximize." Both yield \textit{optimal solutions} that have diametrically opposite utility performance. The best possible and worst possible strategies for a given optimization can both be said to be optimal strategies, if the optimization is tweaked.  A broader and perhaps deeper point is that \textit{any decision can be framed as the solution to an optimization problem}. By limiting the feasible set enough, and framing the objective in just the right way, any number of optimization problems can yield any decision as its optimal solution. Using optimal as justification, then, does not translate to ethical justification by any means. 


==> sections/problems.tex <==
\section{Emergent Problems and Neglect}\label{sec:neglect}

The optimization paradigm requires a number of choices, simplifications, and assumptions, as demonstrated in Section \ref{sec:assumptions}. These choices can contain particular commitments and serve particular interests. A company's goals, priorities, values, norms, and conventions can influence the considerations that end up in an optimization model. As such, `optimal' decision-making in one company or sector means something very particular and context-dependent. A decision described as `optimal' or `optimized' is not, necessarily, a virtuous decision.

Our contention is that optimization is a powerful tool; its use is not ethically neutral simply because it is quantitative and scientific.\footnote{Relatedly, applications of \textit{mechanism design} have been referred to as `technologies of depoliticization' \cite{hitzig2020normative}. See also \citet{Viljoen} and \citet{hitzig2019technological} on mechanism design’s normative dimensions. Mechanism design can be described as a type of optimization and, similarly, can invoke objectivity or impartiality.} Optimization can be used for a number of desirable or undesirable ends, and its application can lead to emergent issues and downstream consequences. We do not argue that optimization’s constituent choices and assumptions are inevitably problematic. Instead, we use the process (or life cycle) of optimization to identify ethical pitfalls, harms, and wrongs that can emerge. 

\subsubsection*{When are these problems `neglected'?} To neglect is to \textit{fail to care for properly}. The worry with optimization is that it can appear to be objective and exhaustive. Optimization is a systematic paradigm used to approach decisions, constraints, and goals, however, its use does not guarantee that all relevant decisions, constraints, goals, interests, values, and other considerations have been adequately weighed. As we describe in this section, there are several cases where optimizations do not properly account for particular harms or values. When an optimization does not take proper consideration of ethically relevant interests or consequences, these interests or consequences may be described as \textit{neglected}.

To be sure, some emergent problems and downstream consequences are unknown and unforeseeable. For example, consequences that are far enough in the future, or that arise from apparent anomalies, may be exceedingly difficult to predict and account for in a decision calculation. These harms and wrongs are difficult to attribute to a lack of care. But, by observing and documenting known problems and failure modes, these cases can inform standards of care and accountability mechanisms.

This section puts forward six emergent issues that can be overlooked when optimization is used to justify or derive a decision. These issues arise at various steps throughout the optimization life cycle. Where relevant, we provide examples and suggestions.

\begin{table*}[htp]
\caption{Breakdown of categories of assumption, neglected problems, and emergent issues in the optimization life cycle.}
\label{table:summary}
\footnotesize
\begin{center}
\begin{tabular}{l l l}
\toprule
% headers
\textbf{Life Cycle Steps} &   \textbf{Neglected Problems}   &   \textbf{Emergent Issues}   \\
\midrule
% [<number>] controls vertical text placement
\multirow{2}[2]{*}{Measurement (\ref{subsec:measure})}   &   \multirow{2}[2]{*}{Label Mismeasurement (\ref{subsec:labelmismeasurement})} &
    % divided row -- first line; this is busted but at least it works
            {Imprecise Labels (\ref{subsubsec:impreciselabels})}      \\
    \cmidrule{3-3}
    % divided row -- second line
    & & Biased Labels (\ref{subsubsec:biasedlabels}) \\
% second super-row
\midrule
% [<number>] controls vertical text placement
\multirow{7}[7]{*}{Modeling (\ref{subsec:model})}   &   \multirow{2}[2]{*}{Problematic Decision Boundaries (\ref{subsec:imprecisedecisionboundaries})} &
    % divided row
            Faulty Modularity Assumptions (\ref{subsubsec:faultymodularity})  \\
    \cmidrule{3-3}
    % divided row -- second line
    &  & Feedback Loops (\ref{subsubsec:feedbackloops}) \\
        
% third super row
\cmidrule{2-3}

   &   \multirow{2}[2]{*}{Neglecting to Consider Multiple Agents  (\ref{subsec:neglectingtoconsidermultipleagents})} & Objective Reflects Narrow Interests (\ref{subsubsec:objectiverepresentsnarrowinterests})  \\
   
   \cmidrule{3-3}
   
   & & Decision Model Formalizes Notions of Control (\ref{subsubsec:decisionmodelformalizes})\\

\cmidrule{2-3}

   &   \multirow{3}[3]{*}{Misspecifying Values (\ref{subsec:misspecifyingvalues})} & Omitting Values (\ref{subsubsec:omittingvalues}) \\
   
   \cmidrule{3-3}
   
   & & Mistakenly Modeling a Value as a Constraint (\ref{subsubsec:mistakenlymodelingconstraint}) \\
   
   \cmidrule{3-3}
   
   & & Mistakenly Modeling a Value as an Objective (\ref{subsubsec:mistakenlymodelingobjective})\\

\midrule
% [<number>] controls vertical text placement
\multirow{2}[2]{*}{Computing (\ref{subsec:compute})}   &   \multirow{2}[2]{*}{Faulty Solution Steps (\ref{subsec:sloppy})} & Faulty Use of Relaxations (\ref{subsubsec:sloppyrelaxations})
    % divided row -- first line; this is busted but at least it works
                \\
    \cmidrule{3-3}
    % divided row -- second line
    & & Faulty Use of Approximation Algorithms (\ref{subsubsec:sloppyapproximation})  \\

% fourth super-row
\midrule
% [<number>] controls vertical text placement
\multirow{2}[2]{*}{Application (\ref{subsec:apply})}   &   \multirow{2}[2]{*}{Using ``Optimal'' as Justification (\ref{subsec:usingoptimalasjustification})} & Justificatory Language (\ref{subsubsec:language})\\
    \cmidrule{3-3}
    % divided row -- second line
    & & Reverse Engineering/Retrofitting (\ref{subsubsec:formal})  
            \\
   
\bottomrule
\end{tabular}
\end{center}
\end{table*}

\vspace{-.1in}
\subsection{Label Mis-measurement} \label{subsec:labelmismeasurement}

Issues in the choice of labels and measurements can lead to undesirable outcomes in the application of optimization. Inaccurate labels exhibit errors whereby there is some characteristic distance between a measurement and a true value. In this section, we discuss two types of label mis-measurement which lead to inaccuracy: imprecise labels and biased labels. These mis-measurements can either be a \textit{conceptual error}, whereby proxies or incorrect labels are used instead of a true underlying value, or a \textit{measurement error}, whereby instruments or empirical methods do not work as expected. Accuracy is comprised of both precision and the absence of bias in measurement--below, we briefly discuss label mis-measurement in terms of these two components.

\subsubsection{Imprecise Labels} \label{subsubsec:impreciselabels} 

Imprecise labels are labels with a high degree of uncertainty or low level of significance. A measurement can be precise and inaccurate if it tends to detect values to a certain level of precision, but those values are consistently biased. A measurement is imprecise when its measurement exhibits significant random error. 

\textit{Example: \textbf{Portfolio Optimization}}. After Harry Markowitz put forward a method to optimally diversify portfolios in such a way that maximizes expected return \cite{markowitz1991foundations, markowitz2000mean}, practitioners who tried applying the method found that it under-performed human decisions and even simple equal-weighting methods \cite{Jobson70}. In an article aptly titled ``The Markowitz Optimization Enigma: Is `Optimized' Optimal?'' \cite{michaud1989markowitz} it was shown that, systematically, assets with the highest measurement error were also those that had the highest expected return. \citet[p 68]{jorion1992portfolio} described the issue: ``A major drawback with the classical implementation of mean-variance analysis is that it completely ignores the effect of measurement error on optimal portfolio allocations ... optimization systematically overweights the assets with the highest estimation errors, hence overstates the true efficiency of the optimal portfolio.''


\subsubsection{Biased Labels} \label{subsubsec:biasedlabels}

Biased labels are consistently inaccurate in a way that predictably and systematically leads to different outcomes for different subjects of an optimization.

\textit{Example: \textbf{Medical Risk Assessment}}. \citet{obermeyer2019dissecting} study a risk prediction algorithm that is used on 200 million Americans annually to optimally distribute health services. The objective function of the risk assessment algorithm trained the algorithm to predict future health \textit{costs} rather than health \textit{needs}, and due to a historical gap in access across race, the risk scores systematically recommended fewer Black patients receive medical resources. Notably, the paper invokes the algorithm's \textit{objective function} in framing its inquiry into the mechanism of bias: ``An unusual aspect of our dataset is that we observe the algorithm's inputs and outputs as well as its objective function, providing us a unique window into the mechanisms by which bias arises'' \cite[p 3]{obermeyer2019dissecting}.

\subsection{Misleading Decision Boundaries} \label{subsec:imprecisedecisionboundaries}

A first step in specifying an optimization model is defining and constraining the \textit{decision variable}. Specifying which variables are freely tunable and which values are feasible lays the roadmap for solving the optimization. Doing so dictates the set of potential outcomes, how the problem may be solved, and, perhaps most importantly, what factors are within vs outside the control of the decision-maker.

Specifying the decision involves assumptions about \textit{who makes the decision} as well as \textit{what power they have over the state of the world}. Making such assumptions risks glossing over the mechanism through which a decision-maker enacts change, and a variety of requisite or related decisions that may be involved. The remainder of this section is devoted to 1) neglectful decision boundaries for synchronous decisions (which arise because of \textit{faulty modularity assumptions}) and 2) neglectful decision boundaries for asynchronous decisions (which can lead to \textit{feedback loops}).

\subsubsection{Faulty Modularity Assumptions} \label{subsubsec:faultymodularity}

It can be simpler or convenient to treat problems as separate optimizations when the number of decisions is too vast. The optimization paradigm makes it very easy to divide and conquer by treating the solution of one optimization as an (unchanging) parameter in a second problem. 

\textit{Example: \textbf{Transit}}.
\bldelete{Consider a metropolitan transit authority faced with the following decisions: Given budget and staff constraints, how many lanes to add to a highway and how much to charge in tolls. In actuality, these decisions are not independent: how much a highway charges in tolls will impact the number of cars on the road, which in turn is important in considering the number of lanes to build. Similarly, how many lanes get built will constrain how many people will commute by car and significantly affect budget and revenue considerations for the toll decision. A potentially inadequate way of making this decision would be to treat each choice as independent: first, decide how many lanes would serve the population, and then (conditional on a set number of lanes) decide what to charge in tolls. \bldelete{The road gets built once and typically does not add or remove lanes for long periods of time. After construction, states may choose to charge tolls, and would consider the number of lanes as a constraint while they optimize for particular objectives–for example, traffic throughput and revenue.} Instead, sophisticated methods for simulating road use might enable traffic engineers to better understand the interplay between their various decisions, thus leading to transportation designs that serve people. 
}
\tgedit{Consider a metropolitan transit authority faced with the following decisions: given budget and staff constraints, how much to charge in tolls and whether (or which) lanes should be restricted to high-occupancy vehicles during peak travel times. In actuality, these decisions are not independent: how much a highway charges in tolls will impact the number of cars on the road by inducing demand, which in turn is important for evaluating to what extent high-occupancy vehicle lanes will improve overall traffic throughput. Similarly, how many lanes will be restricted---or the window of time during which the restriction is enforced, or how costly the fine---will constrain how many people may commit to carpooling and significantly affect budget and revenue considerations for the toll decision. These choices could be treated in isolation: first, decide how many restricted lanes would serve the carpooling population, and then (conditional on a set number of lanes) decide what to charge in tolls. But to do so would ignore the fundamentally interdependent nature of the decision, and may generate spillover effects that the simplistic model does not account for.}

\textit{Using the Handoff Framework} Imprecise decision boundaries, including incorrect assumptions about modularity, lead to short-sighted optimizations that may not serve the broader function of a system, or may lead to grave risks or emergent harms. Anticipating, diagnosing and confronting these harms requires an understanding of the normative implications of exchanging or improving component parts of a complex socio-technical system. For this kind of inquiry, the theory of \textit{\textbf{handoff}} \cite{mulligan2020concept,goldenfein2020through} provides a useful account of how divide-and-conquer optimization strategies, with incorrect modularity assumptions, can have unanticipated normative and political implications. \citet[p 245]{mulligan2020concept} use the example of access control to illustrate this point: although tech companies can justify switching from passwords to fingerprints to face ID by saying each new technology more \textit{optimally} performs the specified function of access control, such changes have notable political implications; for instance each successive handoff might be said to curtail user control and diminish transparency. Handoff suggests that improving these sub-functions without considering broader normative implications is not sufficient justification for exchanging or updating a technological sub-component.

\subsubsection{Feedback Loops} \label{subsubsec:feedbackloops}

Optimizations may arise in a repeated fashion where it is unreasonable to assume each sequential decision is independent. For the same reason numerous synchronous decisions may be haphazardly split into separate optimizations (discussed in Section \ref{subsubsec:faultymodularity}), modelers may unreasonably assume sequential decisions are independent.

The phenomenon of feedback in optimization is represented in Figure \ref{fig:lifecycle}'s depiction of the entire optimization life cycle as a loop. Optimizations can be used repeatedly, even if the formal operational strategy does not account for one optimization’s impact on the next. Similar feedback loops have been observed in statistical systems that do not necessarily involve optimization – in domains ranging from mechanisms and acoustics to economic inequality, the concept of feedback and path-dependence explains patterns where compounding or overlapping impacts from multiple sequential events lead to unanticipated or chaotic events. In the context of fairness for socio-technical systems, \citet[p 62]{selbst2019fairness} described this phenomenon (and corresponding neglect on behalf of designers) as the \textit{ripple effect trap}.

 In the case of optimization, it may be that an optimal decision in one instance is sub-optimal or actively harmful when repeated sequentially over time. A common example of this difference comes from bad modeling set-up or incorrect assumptions can lead an agent to so-called `greedy' policies where they always exploit known reward, or always explore new and high-risk options (see e.g. \cite{bubeck2009pure}). \textit{Multi-armed bandit} problems \cite{bubeck2012regret, vermorel2005multi, lu2010contextual} reflect this dynamic: knowing that an agent has many decisions that can be made in sequence, it may be optimal to explore new unknown choices. Agents with only one decision, however, may instead opt to exploit their known option with the highest value.
 
\textit{Example: \textbf{Predictive Policing}}. The tendency to \textit{exploit} when sequential optimizations are treated as individual decisions has been shown to cause harmful disparities in treatment. To illustrate this point, consider the example of PredPol (now re-branded as Geolitica), a commercial predictive policing software that used historical data to statistically train optimal\footnote{i.e., the predictive algorithm developed by PredPol used expectation-maximization techniques developed in \cite{mohler2014marked}, as noted in \cite{mohler2015randomized} and \cite{ensign2018runaway}.} policing recommendations \cite{mohler2015randomized}. The software was accused of formalizing and entrenching historical biases \cite{lum2016predict, isaac2017hope, silva2018algorithms}. Theoretical models of sequential predictive decisions provided an explanation for these emergent biases: Predictions made as single-shot optimizations can introduce \textit{runaway feedback effects} when applied sequentially over time, since predictive algorithms direct police to neighborhoods where crime was historically observed \cite{ensign2018runaway, laufer2020compounding}.

\subsection{Neglecting to Consider Multiple Agents} \label{subsec:neglectingtoconsidermultipleagents}

A notable feature of optimization is its strict delineation between decision variables and other (non-decision) variables: Certain parameters are considered to be in the control of the decision-making agent, and other parameters are exogenous and outside the direct control of the agent. This approach makes it convenient to divide optimizations into individual, simple decisions as described in Section \ref{subsec:imprecisedecisionboundaries}. The approach also lends itself to treating decisions as belonging to a \textit{singular agent}. Even though optimizations are commonly used by institutional bodies and passed between numerous stakeholders ranging from analysts to engineers to executives, these optimizations may not consider that the various constituents of an organization are distinct decision-makers themselves. In this section, we consider how optimization problems may neglect to properly consider the agency of multiple decision-makers, and how such neglects can be avoided or identified. When multiple agents are not taken into consideration, optimizations may only serve the interests of a few people, and additionally may codify or formalize particular structures of management and control. In this section, we consider each of these emergent issues. 

\subsubsection{Objective Represents Narrow Interests} \label{subsubsec:objectiverepresentsnarrowinterests} Optimization is used to make logistical decisions that can impact many people, both inside and outside the decision-making apparatus. For a given optimization, the relative importance of different agents’ utility can be defined in the objective function. When an objective omits or de-values harmful impacts on certain populations, the resulting ``optimal'' decision can be ethically wrongful.

When an objective reflects only certain interests in an organization, the optimal decision might justify exploitative working conditions. Take the toy example of a board of directors deciding how to use a certain amount in earnings. Without union representation on the board, they might decide that their utmost priority is to keep investors happy and therefore pay dividends. With union representation, however, they might adjust their priorities and devote more earnings to employee compensation. The choice of \textit{goal} or \textit{objective} is highly dependent on the organizational structure.\footnote{We refer readers to \citet{kasy2021fairness}, which puts forward a formal notion of \textit{power} as it relates to designing the objective function.}

\textit{Example: \textbf{Technology Adoption}}. When financial mathematicians began to suggest that optimization could improve portfolio diversification schemes, firms were slow to adopt these schemes. In one academic paper devoted to the reasons why firms did not adopt these measures, a reason for the resistance was the social and political structure of the firm: ``Probably the single most important reason why many financial institutions don't use portfolio optimizers is \textbf{political}. This is because the effective use of an optimizer mandates significant changes in the structure of the organization and the management of the investment process'' \cite[p 32]{michaud1989markowitz}. Firm managers did not want to cede decision-making power to quantitative analysts, suggesting internal organizational social structure influences the use of optimization. 

\ 

The ``narrow interests'' described so far concern internal social structures in a decision-making apparatus. But problems of narrowly defined goals can also have massive impacts on people external to the decision who have little or no relation to the particular company or institutional body's decision. The notion of \textit{externalities} \cite{ayres1969production, baumol1972taxation, cornes1996theory} (see also \cite{coase2013problem}) from economics helps to describe how unaccounted-for impacts can affect people who might face barriers entering into contracts or fending off negative consequences. People downstream from a river might be negatively impacted by factory pollution and may not even know it. These effects can be the result of negligent or malicious tweaks to an objective function. They highlight the importance of critically evaluating optimizations and their stated goals.

\subsubsection{Decision Model Formalizes Notions of Control} \label{subsubsec:decisionmodelformalizes} Moving beyond how the objective is defined, the \textit{decision variables} in an optimization are an important indicator for what an agent has control over. In formalizing exactly what decision is assumed to be under the control of an agent or organization, an optimization can codify existing social structures.

\textit{Example: \textbf{Workforce Optimization}}. Industries are fiercely competitive over employee talent, and retaining employees has become an important priority for companies. So-called `workforce optimization' \cite{roy2019enabling, naveh2007workforce, altner2018two} or `staff planning problems' \cite{anderson2001nonstationary, balachandran1982interactive, abernathy1973three} devise strategies to allocate, promote and pay workers in order to maximize retention and efficiency while minimizing employer costs. Such models make assumptions about a particular type of employee/employer relationship, for example that employees are contractors whose time can be allocated freely; or that layoff recommendations can come from performance metrics rather than human judgments. The clearest examples of decision models formalizing or implicating systems of control are warehouse management and logistics studies that create staffing tools for warehouse managers that balance worker discomfort, worker risk, and efficiency \cite{wruck2017risk, larco2017managing}.\footnote{These tools are further discussed in \cite{gong2011review, de2017warehouse}.}

\subsection{Mis-specifying Values} \label{subsec:misspecifyingvalues}

Optimization requires formally specifying at least one decision and at least one notion of value or utility. The values laden in optimization are made most apparent by the existence of an objective function, which formalizes a goal or certain measure of utility that the decision-maker is assumed to wish to maximize. But values play into a number of other aspects of a model as well: Models often include constraints motivated by ethical norms or values like fairness.

In this section, we discuss the issues that arise when a model is mis-specified in such a way that values are not given rightful consideration. We contend that there are two mechanisms that result in mis-specified values: 1) leaving values out of an optimization completely and 2) mistreating or mis-modeling values within an optimization. In discussing the latter type of mis-specification, we consider instances where values are wrongfully incorporated as optimization constraints (instead of objectives), or wrongfully incorporated as objectives (instead of constraints). 

\subsubsection{Omitting Values} \label{subsubsec:omittingvalues}

Omitting values from an optimization problem can be either negligent or deliberate. A negligent omission of values arises when the humans designing and executing an optimization are unaware of the ramifications of their modeling or measurement assumptions. For example, a company that makes custom shirts might decide where to source their textiles. An optimization problem that minimizes the cost of textiles might suggest changing which factory they contract with. However, it could be that the new factory has dangerous working conditions or otherwise harsh and unethical labor policies. If the optimization designer was unaware of this distinction, the omission of labor considerations from the decision would be \textit{negligent}; if they were aware, it would be \textit{deliberate}.

Scrutinizing which values and implications are included or excluded from an optimization provides important information for attributing harms and establishing \textit{\textbf{accountability}}, but one can not differentiate negligent and deliberate omissions from the optimization model alone–further contextual evidence is needed to qualify the human decisions behind an optimization model. In the case that a value is omitted from an optimization on purpose, agents may use the optimization's output as \textit{justification} for a certain decision. We turn back to this idea in Section \ref{subsec:just}.

\subsubsection{Mistakenly Modeling a Value as a Constraint} \label{subsubsec:mistakenlymodelingconstraint}

Often a constraint is added to a model which is based on a moral imperative: A new housing development in a lower-income neighborhood may be required to reserve a certain number of units as rent-stabilized, low- or middle-income housing, leading developers to treat this requirement as a constraint on building a profitable new development. When companies boycott sales in foreign areas to voice dissatisfaction with states’ political decisions, their resulting business strategy is constrained by their stance; even if their supposed goal is profit and expansion. When somebody decides to go on a diet and cut out added sugars, similarly, they approach their food decisions with constraints because resetting the objective may be more difficult to hard-wire.

These values are assumed to be categorical, rules-based, and violating them becomes fully infeasible when they are incorporated as a constraint. Values such as \textbf{\textit{fairness}} are assumed to be constraints, even though concepts such as \textbf{\textit{equity}} may readily be considered utilities to be maximized. Though constraints play an important role in determining the feasible set of decisions available to a decision-maker, they can also be weak in guiding values judgments: As long as a decision is feasible, constraints play no role in preferring one decision over another. So, within the feasible set, a constraint has no bearing on what option gets chosen. What's more, non-negligible constraints that are added to an optimization tend to yield solutions that lie on these constraints: \textbf{\textit{solutions tend to `bump up against' constraints.}} In practice, this can mean that `optimal' solutions do the \textit{bare minimum} at meeting some values-driven imperative.

\textit{Example: \textbf{Access}}. Consider a city which has two potential ways of providing transportation to its people. One option is to allow private industry to provide transportation through contracts with the city. In this case, providers might reach decisions with the city that constrain their behavior, for instance that they must provide a certain level of access to low-income neighborhoods. At the end of the day, however, their objective is to \textit{maximize profit} subject to \textit{legal constraints}.  An alternative option is to treat transportation as a public service, where a single entity with a budget is tasked with providing transportation. In this public approach, an agency might aim to \textit{maximize access} subject to \textit{budgetary constraints}. These two approaches to optimization logic encode the same values (access and budgetary responsibility) but do so in ways that can lead to vastly different levels of access across communities.

\subsubsection{Mistakenly Modeling a Value as an Objective} \label{subsubsec:mistakenlymodelingobjective}

An objective function defines utility as a quantifiable and measurable function of the relevant decision $x$. This way, for any particular decision value $x_i$, the utility of that decision can be directly compared (via a quantitative scale) to an alternative decision $x_j$. Defining the objective lends itself well to \textit{ends-based} or \textit{utilitarian} frameworks\footnote{Quantification and prediction are key facets of utilitarianism, which as an ethical project aims to maximize utility. A relevant paper which discuss the theme of operationalization and utilitarianism is \cite{zame2007can}.} which treat value as quantifiable and to some extent predictable \cite{sinnott2003consequentialism}. In fact, an optimization model presumes to model the relationship between a decision and its utility outcome---in non-stochastic optimizations, this relationship is presumed to be fully known and defined, whereas stochastic optimization models randomness explicitly \cite{sahinidis2004optimization}. Sometimes, values are treated as objectives when they ought to be modeled elsewhere in an optimization. These instances tend to involve misplaced incentives---a company is incentivized to maximize profit, even if they should really be incorporating other notions of utility in their optimization. 

\textit{Example: \textbf{Safety}}. Car companies communicate that they aim to build the safest cars. In reality, these companies have many goals including engine efficiency, speed, comfort, and profit. If safety were truly the utmost objective, a car would not move: staying parked is the safest state for a car. Of course, the functionality of a car requires that safety is not always modeled as a \textit{sole} objective (even if such an objective is communicated in advertisements). More realistically, many car companies' safety considerations are treated as \textit{constraints}.\bldelete{ A similar case can be made for telecommunication companies’ relationship to \textit{\textbf{privacy}}---the devices and networks created functionally create ramifications for privacy; and optimizing for privacy alone would be futile.}

\subsection{Faulty Solution Steps} \label{subsec:sloppy}

The steps involved in solving an optimization problem, from relaxations to iterative algorithmic solutions, involve assumptions and simplifications that ought to be dealt with carefully and notated precisely. In this section, we discuss two types of neglect in the steps involved with solving optimizations: \textit{faulty use of relaxations} and \textit{faulty use of approximation algorithms}. Our goal in this section is not to critique optimization research, which tends to precisely and clearly characterize the use of approximations, nor to critique all applications of optimization. More often, these areas of neglect can occur in private settings which emphasize speed and minimum viability \cite{ries2009minimum, moogk2012minimum} in product development.

\subsubsection{Faulty Use of Relaxations} \label{subsubsec:sloppyrelaxations}

When a relaxation is used for ease of computation or measurement, it can significantly change the optimization's feasible set and objective function.  As such, it is important to detail when relaxations are being used, and what assumptions are made in the process. When a problem is relaxed, its fundamental structure has changed. The solution set might be much bigger, or smaller, than the true optimization problem, for example. As such, calling a solution to a relaxed problem `optimal' may be misleading without appropriately caveating. When relaxations are purposefully concealed and a solution is described as \textit{optimal}, such a practice is \textit{faulty}. It postures as \textit{legitimate} on false pretenses, even when its recommended choice could be mis-guided or non-optimal.

\subsubsection{Faulty Use of Approximation Algorithms} \label{subsubsec:sloppyapproximation}

It is common for operations researchers, mathematicians, and computer scientists to focus on a particular category of problem, come up with a way of approximating the solution, and prove that the approximate solution is within a certain error bound compared to the true solution. In optimization, maximization (minimization) problems are approximated with answers that perform below (above) the true optimal, in which case lower (upper) bounds are given. Approximations are applied haphazardly when these guaranteed bounds are not given, and the performance guarantee or bound is not specified. Approximation algorithms are also applied sloppily if they are derived for a certain \textit{type} of problem (e.g., convex) and are applied on a different type of problem (e.g., non-convex). Such a behavior can be \textit{faulty} when performance is purposefully over-stated, or uncertainty is concealed.

\subsection{Using “Optimal” as Justification} \label{subsec:usingoptimalasjustification} \label{subsec:just}

The final problem identified in this paper arises when people assume that an \textit{optimal decision} is an \textit{ethically justified decision}. As optimization has entered common parlance, it is used to describe a variety of behaviors and strategies that aim to achieve a variety of ends. Optimization is sometimes invoked without specifying a particular decision or objective---an optimal workforce strategy or an optimal economic policy lack the kind of specificity that is required to understand if a particular strategy is morally or politically desirable. In this section, we discuss the justificatory use of optimization. Particular mechanisms by which optimization can be used to justify action are apparent in language (e.g., when a decision-makers calls their decision \textit{optimal} without further context) and in cases where an optimization problem is retrofit to a decision that has already been made.

\subsubsection{Implicit Subject-Object Relationship} \label{subsubsec:language}

The use of the verb ``optimize,'' when used in the sense we discuss in this paper, implies that there is a \textit{decision} and a \textit{goal}. Sometimes, when people use the word without specifying one of these constitutive components, the context can clarify: ``optimize draft picks" might specify the decision and imply the goal, for example. When the decision and goal are indeterminate and a quantity is claimed to be \textit{optimal}, however, we argue that this description is a category error and its use is a primary suspect for the sort of neglect we are describing. Especially in high-stakes settings, where the goals of a certain decision might be contested, such as admissions, sentencing, and urban policy, using the word \textit{optimal} to describe a particular decision may be a faulty justification or optic maneuver.

\blcomment{\paragraph{Example: ?} Example}

\subsubsection{Reverse Engineering} \label{subsubsec:formal}
Beyond the \textit{linguistic} use of optimization to justify behavior, we make a slightly stronger claim: even if an optimization model is defined and solved indicating that a particular decision is optimal, such a process does not morally justify making that decision.  This point can be demonstrated by considering two optimizations, nearly identical, except one switches ``minimize" for ``maximize." Both yield \textit{optimal solutions} that have diametrically opposite utility performance. The best possible and worst possible strategies for a given optimization can both be said to be optimal strategies, if the optimization is tweaked.  A broader and perhaps deeper point is that \textbf{\textit{any decision can be framed as the solution to an optimization problem}}. By limiting the feasible set enough, and framing the objective in just the right way, any number of optimization problems can yield any decision as its optimal solution. Using optimal as justification, then, does not translate to ethical justification by any means. 

\blcomment{Potential example:

\textit{Example: \textbf{School Choice}}.

Shi on school choice \cite{shi2015guiding}

Hitzig on school choice \cite{hitzig2020normative}
 }

==> sections/programme-new.tex <==
\section{Discussion and Suggestions}\label{sec:programme}

Optimization is a paradigm used to aid and support decision-making in potentially high-stakes situations. It offers a systematic way of balancing interests and considerations as objectives or constraints relevant to a particular decision. The required design choices --- including which interests and considerations to model, and how to model them --- are often guided by norms, commitments and priorities. For example, a social media company might use optimization to recommend content in a way that attracts attention and engagement from users. Or, a government might use optimization to set tariffs in a way that promotes growth while satisfying domestic workers and unions. Using optimization in a particular domain requires making choices not just about which factors to include, but also about which factors to omit. Much of the context around a decision is omitted in order to model the decision as an optimization. Accordingly, when an optimization is “solved” and a course of action is selected, this does not suggest that the action is morally or ethically or socially good, \textit{all things considered}. Instead, the so-called `optimal' solution satisfies a very specific set of considerations: namely, those that are specified and introduced through the process of modeling, measuring, computing and applying the paradigm.

In this paper, we put forward a framework for understanding the normative commitments that are contained, either implicitly or explicitly, in the use of mathematical optimization. To do so, we focused on the steps involving abstraction and assumption, many of which are choices that reflect practitioners’ priorities and values. We then attempted to excavate some of the assumptions, areas of neglect, and emergent issues that can arise along the various components of an optimization’s life cycle. 

As researchers are reckoning with the potential for bias, unfairness, inequality, opacity, and other ethical issues in machine learning and dataset creation, a similar line of inquiry is needed to scrutinize the normative (and epistemic) elements of optimization. A number of research questions in this line of inquiry remain, including: which norms, commitments, and priorities might constitute appropriate or legitimate optimization?

These and other considerations around optimization and optimal behavior are open questions that, we hope, will motivate a program of future research. There are a number of directions for work, some of which stem directly from the present paper’s framework.

\textit{Empirical work}. The use of optimization as a paradigm for decision-making requires constructing an abstract model and using it to make decisions in real-world contexts. Empirical studies about optimization’s use and impacts may find particular patterns, conventions, and mechanisms through which optimization causes social harms (or, conversely, benefits). Sometimes, simply observing and documenting the components of an optimization (e.g., the objectives) can provide useful empirical insight about an individual or institution’s operations. For example, the fact that a social media company designs features to optimize for user engagement and attention might reveal pressing and legitimate issues about its products.

Available traces and artifacts pointing to the use of optimization are crucial for empirical study and, ultimately, conversations about appropriate use. To that end, \textit{documentation} can play a role in making optimization use transparent and accountable. The work on documenting models \cite{mitchell2019model}, datasets \cite{gebru2021datasheets}, and reinforcement learning models \cite{gilbert2022reward} might hold lessons for optimization. These studies can ultimately enable audits, new standards, best practices, and other mechanisms for accountability.

\textit{Conceptual work}. This paper provides evidence that optimization is a paradigmatic technical tool that encodes certain normative commitments. Theorizing about whether and when these commitments are justified remains a promising direction for further inquiry. Normative analysis of this sort might benefit from careful consideration of a number of contextual parameters about the use of optimization: By whom? Of what? When? Where? For what end? They may also benefit from a more aggregate and system-wide framing on optimization and its political implications. For instance, it seems evident that private corporations tend to optimize for profit, or a proxy thereof. In light of this, how can markets, institutions and processes improve the use of optimization and aim technological tools towards social ends?

==> sections/programme.tex <==
\section{Discussion and Suggestions}\label{sec:programme}

In this paper, we put forward a framework for understanding the normative implications of optimization modeling. We began with a model for understanding the sequential steps in an optimization design and execution and proceeded to excavate the assumptions, areas of neglect, and emergent issues that can arise in such a life cycle. 

Further research is needed to understand, diagnose, and scrutinize the use of optimization in a wide variety of domains. As researchers are reckoning with the potential for bias, unfairness, inequity, opacity, and other ethical issues in machine learning and dataset creation, a similar line of inquiry, equipped with our framework, might illuminate harms that arise in operational uses of optimization. Ultimately, our work is intended to add precision to empirical inquiries about the use of optimization and its downstream impacts. The FAccT community is particularly well-positioned to conduct empirical studies about where biases, harms, and risks get introduced to the optimization framework, given its interdisciplinary focus and substantive connections across the landscapes of industry, policy, and research.

When addressing social problems, computational researchers may fill various roles that interface with longstanding patterns of injustice and inequality \cite{abebe2020roles}. In particular, there is a need for optimization practitioners to reflect on the relationship between these roles and what is expected of their own mathematical techniques within\bldelete{a given Machine Learning pipeline} any particular product life cycle. Pierre Bordieu's notion of \textit{reflexivity} \cite{bourdieu2004science} suggests that critical self-evaluation is necessary in social-scientific scholarly fields---this invitation \cite{bourdieu1992invitation} has already been taken up by a number of ML-ethics researchers (see e.g. \cite{miceli2021documenting, laufer2022four, elish2018situating}). Reflection is needed so that normative concerns are able to be addressed and interrogated (rather than neglected) in the course of a given optimization approach. In some cases, such an interrogation may motivate the adoption of a different approach altogether. Below, we briefly present two research practices that, if widely adopted, would make reflection about the terms of optimization both possible and technically tractable.

\textit{Context-Sensitive Empirical Methods}: Since optimization is highly context-dependent, empirical studies about optimization's use and downstream impacts may require new observation studies and modes for data collection. In industry settings, optimizations aid in managerial decisions and in setting core business parameters; their use may be instrumental in meeting \textit{key performance indicators} (KPIs) or \textit{Objects and Key Results} (OKRs), terms related to the \textit{objective} familiar to optimization researchers. The relationship between available sources of data, business decisions, KPIs and OKRs might be best expressed when optimizations are written out or systematically tracked.\bldelete{ However, it may also be that optimizations are developed in iterative processes (in the presence of feedback), so that formal optimizations are written out only a few times throughout an analysis, or after the decision has been made, or not at all. It may be fruitful to consider what an explicit approach to problem formulation would entail for the impacts and assumptions laden in this process.}

The empirical methods that would aid in future research on the use and mis-use of optimization include \textit{qualitative} and \textit{quantitative} methods. On the qualitative front, treating the code, documentation, and other artifacts in optimization as data, social scientific inquiry might yield generative conclusions about the goals, priorities, and inner workings of organizations that employ optimization. On the quantitative front, causal statistical methods might link downstream harms of optimization to modeling steps in the optimization life cycle. 


\bldelete{A given problem may have several Pareto-optimal solutions \blcomment{we do not discuss this in the paper as of now}. In industry settings, these choices are often handed to a manager or executive who evaluates which is most desirable in light of key performance indicators (KPIs), or even more abstractly, Objects and Key Results (OKRs). Often the relationship between available sources of data, KPIs, and OKRs is implicit in the feedback loop that structures optimization problems. Indeed, it may be that optimizations are written after an analysis has been completed, or not written out at all, in many industry contexts. However, it is interesting to consider what an \textit{explicit approach} to problem formulation would entail for the impacts and assumptions laden in this feedback loop. In that case, a variety of empirical methods could be useful in further studies related to the impacts and assumptions laden in optimization. More specifically, a variety of qualitative sociological methods may be useful for investigating the real-world assumptions that underline optimization problems once they have been completely written out, as these documents would have to outline various normative considerations that may or may not hold empirically. It would be useful to investigate exactly what gets optimized in a variety of industries when a Machine Learning task is understood in relation to KPIs and OKRs. For example, in what ways is a social media recommender optimizing for shareholder profit vs. user engagement in the context of the tech firm's wider business model? In addition, econometric and causal methods about the downstream harms of executing an optimal decision-process, as done in some papers already [e.g. Obermeyer on Health risks, etc] \blcomment{needs attention}, could use and build on our framework.}

\textit{Documentation}: The framework proposed in this paper may enable reflection on the proper sorts of documentation for the transparent and accountable use of optimization in practice. Following leading work on documenting model performance \cite{mitchell2019model, shen2021value} and dataset creation \cite{gebru2021datasheets},\footnote{We also refer the reader to work on audits \cite{ajunwa2019auditing, raji2020closing}, annotations \cite{raji2019ml, beretta2021detecting}, impact assessments \cite{metcalf2021algorithmic, moss2021assembling, metcalf2022relationship}.} we propose that similar work might be useful for anticipating and documenting the use of a particular optimization frame or algorithm. One recently proposed framework calls for \textit{Reward Reports}, which are intended to support a dynamic understanding of equity and access with reference to both what a given system is optimizing for and its observed behavior over time \cite{gilbert2022reward}. A documentation approach of this sort by no means guarantees accountability, which is a contested and relational notion requiring significant policy infrastructure \cite{wieringa2020account, bovens2007analysing, cooper2022accountability}. However, dynamic and intervention-specific forms of documentation could proactively align the intentions and consequences of various optimization techniques, making it easier to anticipate harms and providing grounds for liability in high-stakes settings \cite{mehta2023dynamic}.

\ 
